Exploiting the Asymmetric Uncertainty Structure of Pre-trained VLMs on the Unit Hypersphere

Vision-language models (VLMs) as foundation models have significantly enhanced performance across a wide range of visual and textual tasks, without requiring large-scale training from scratch for downstream tasks. However, these deterministic VLMs fail to capture the inherent ambiguity and uncertainty in natural language and visual data. Recent probabilistic post-hoc adaptation methods address this by mapping deterministic embeddings onto probability distributions; however, existing approaches do not account for the asymmetric uncertainty structure of the modalities, and the constraint that meaningful deterministic embeddings reside on a unit hypersphere, potentially leading to suboptimal performance. In this paper, we address the asymmetric uncertainty structure inherent in textual and visual data, and propose AsymVLM to build probabilistic embeddings from pre-trained VLMs on the unit hypersphere, enabling uncertainty quantification. We validate the effectiveness of the probabilistic embeddings on established benchmarks, and present comprehensive ablation studies demonstrating the inherent nature of asymmetry in the uncertainty structure of textual and visual data.

==> asymvlm_latex/sec/abstract.tex <==
\begin{abstract}
Vision-language models (VLMs) as foundation models have significantly enhanced performance across a wide range of visual and textual tasks, without requiring large-scale training from scratch for downstream tasks. However, these deterministic VLMs fail to capture the inherent ambiguity and uncertainty in natural language and visual data. Recent probabilistic post-hoc adaptation methods address this by mapping deterministic embeddings onto probability distributions; however, existing approaches do not account for the asymmetric uncertainty structure of the modalities, and the constraint that meaningful deterministic embeddings reside on a unit hypersphere, potentially leading to suboptimal performance. In this paper, we address the asymmetric uncertainty structure inherent in textual and visual data, and propose AsymVLM to build probabilistic embeddings from pre-trained VLMs on the unit hypersphere, enabling uncertainty quantification. We validate the effectiveness of the probabilistic embeddings on established benchmarks, and present comprehensive ablation studies demonstrating the inherent nature of asymmetry in the uncertainty structure of textual and visual data.
\end{abstract}

==> asymvlm_latex/sec/asym_structure.tex <==
\section{Asymmetric structure of texts and images}\label{sec:asym}
The relationship between vision and language exhibits an inherent asymmetry in its uncertainty structure. A textual concept, such as "dog," acts as an abstract type that can map to a vast number of unique real-world instances (tokens). Each of these instances can, in turn, be captured in countless images differing in viewpoint, lighting, and composition. This cascaded one-to-many mapping—from abstract type to physical token, and from token to specific image—induces high aleatoric uncertainty in the text modality.

Conversely, an image portrays a single, specific token. While it depicts one object unambiguously, it can be described by multiple valid captions (e.g., "a dog," "a golden retriever," "a pet"). This one-to-many mapping, from image to text, arises from linguistic diversity. Therefore, the uncertainty in text-to-image retrieval (rooted in abstraction and visual variability) is fundamentally different from that in image-to-text retrieval (rooted in descriptive variance). Despite this structural asymmetry as shown in Figure \ref{fig:diagram}, existing post-hoc probabilistic adapters typically treat both retrieval directions symmetrically.

% In linguistics and semiotics, the relationship between words and objects is often described as the type–token-distinction \cite{wetzel2009types}: the word "dog" is a type (an abstract label applicable to any dog), whereas a single dog is a token (a specific instance). Textual labels are high-level abstractions, and can map onto infinitely many unique physical examples. In contrast, a single dog is one particular realization of the word "dog". However, for the single dog, infinitely many images can be taken with different setups, e. g., different angles, color tones.
% The one-to-many and many-to-one mappings from the text and vision to physical world, respectively, imply the intrinsic asymmetric structure in textual and visual information. This is of vital importance for the understanding cross-modal retrieval, and subsequently the building of VLMs. 

% Crucially, text and images exhibit different kinds of one-to-many ambiguity (Fig. \ref{fig:diagram}). The word "dog" can denote any of infinitely many dog instances (objects), each of which can in turn be photographed under many viewpoints, lighting conditions, etc. Thus text$\to$object is one-to-many via abstraction, and object$\to$image is one-to-many via visual variability. In contrast, a photo of a golden retriever unambiguously depicts one physical object but admits multiple valid captions (e.g., "a golden retriever,", "a dog," "an animal"). Thus image$\to$text is one-to-many through diverse linguistic descriptions. Existing post-hoc probabilistic adapters treat these two retrieval directions symmetrically.

\begin{figure}[t]
% \vspace{0.5\shrinklength}
    \centering
    \includegraphics[width=\linewidth]{figures/asymvlm_diagram.pdf}
    \vspace{\shrinklength}
    \caption{Asymmetric probabilistic adaptation (AsymVLM): Texts are encoded with a frozen text encoder and adaptor to produce probabilistic hyperspherical embeddings (e.g., vMF distribution), while image are deterministically encoded via a frozen image encoder. The log likelihood matrix $L$, with element $L_{m,n}$ representing the log likelihood of image vector $z_n^I$ given text embedding $\bm{z}_m^T \sim P(\mu_m, \kappa_m)$, is optimized using InfoNCE to maximize diagonals and minimize off-diagonals.}
    \label{fig:asym_structure}
    \vspace{\shrinklength}
\end{figure}

\subsection{Mathematical formulation}
Let $\mathcal{T}$, $\mathcal{I}$, $\mathcal{O}$ and $\widetilde{\mathcal{O}}$ denote the text, image, (real-world) object and (numerical) representation space respectively. The relationships between $t\in\mathcal{T}, i\in\mathcal{I}, o\in\mathcal{O}$ and $\tilde{o}\in\widetilde{\mathcal{O}}$ can be presented as follows.
\begin{table}[h]
% \vspace{0.5\shrinklength}
% \scriptsize
\footnotesize
\centering
% \caption{Mappings between text, objects, and images.}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{@{}ll@{} c}
\toprule
\textbf{\textsc{Mapping}} & \textbf{\textsc{Definition / Derivation}} & 
\textbf{\textsc{One-to-many?}}\\
\midrule
Text $\to$ Object 
& $\Phi_T(t) \coloneqq \{ o \in \mathcal{O} : o \text{ can be described by } t \}$ & \checkmark \\
Object $\to$ Image 
& $\Phi_I(o) \coloneqq \{ i \in \mathcal{I} : i \text{ is an image of } o \}$ 
& \checkmark \\
Text $\to$ Image 
& $(\Phi_I \circ \Phi_T)(t) = \bigcup_{o \in \Phi_T(t)} \Phi_I(o)$ &
\checkmark\\
\midrule
Image $\to$ Object 
& $\Phi_I^{-1}(i) \coloneqq o$ \quad & \xmark (assumption)\\
Object $\to$ Text 
& $\Phi_T^{-1}(o) \coloneqq \{ t \in \mathcal{T} : o \text{ can be described by } t \}$ & \checkmark\\
Image $\to$ Text 
& $(\Phi_T^{-1} \circ \Phi_I^{-1})(i) = \{ t \in \mathcal{T} : \Phi_I^{-1}(i) \in \Phi_T(t) \}$ & \checkmark\\
\midrule
Object $\leftrightarrow$ Representation & $\psi(o) \coloneqq \tilde{o}, \ \psi^{-1}(\tilde{o}) = o$  & \xmark\\
Text encoder & $f_T \approx \psi \circ \Phi_T$ & \checkmark\\
Image encoder & $f_I \approx \psi \circ \Phi_I^{-1}$ & \xmark\\
\bottomrule
\end{tabular}
\vspace{\shrinklength}
\end{table}

\paragraph{Building VLMs}
Existing datasets such as MS-COCO \cite{coco_dataset} and Flickr30K \cite{flickr_dataset} collect data in the form of $\{(t_n, i_n)\}_{n=1}^N$ such that there exist $o_n\in\mathcal{O}$ which satisfies $o_n \in \Phi_T(t_n)$ and $i_n\in\Phi_I(o_n)$. Based on such datasets, we aim to find a $d$-dimensional real-valued representation space $\widetilde{\mathcal{O}}\subset\mathbb{R}^d$, such that there exists a bijective function $\psi:\mathcal{O}\to\widetilde{\mathcal{O}}$. More importantly, the goal is to approximate the composite function $\psi \circ \Phi_T: \mathcal{T}\to \mathcal{P}(\widetilde{\mathcal{O}})$ and $\psi \circ \Phi_I^{-1}: \mathcal{I}\to \widetilde{\mathcal{O}}$ with finite samples from datasets as the text encoder $f_T$ and image encoder $f_T$, following the Platonic representation hypothesis \cite{huh2024platonic}.

\subsection{Motivating the approach}
% Although both text-to-image and image-to-text retrieval are characterized as one-to-many mappings, their underlying structures differ fundamentally. In text-to-image retrieval, the one-to-many relationship arises from two factors:  the inherent abstraction in textual representations ($\Phi_T$) and the variability of images corresponding to a fixed object ($\Phi_I$). In contrast, image-to-text retrieval entails the one-to-many mapping being attributed to the multiplicity of textual descriptions available for a given object (i.e., only $\Phi_T^{-1}$ is one-to-many). We therefore hypothesize that the ill-posed nature of both tasks originates from this intrinsic asymmetry between text and image information.

Trained on datasets in the form of $\{(t_n, i_n)\}_{n=1}^N$, existing deterministic pre-trained models maximize the similarity measure between matching text-image pairs while minimizing it for non-matching pairs \cite{clip, zhai2023sigmoid}. These approaches effectively learn a real-valued embedding space $\widetilde{\mathcal{O}}$, along with deterministic text and image encoders. Existing probabilistic adaptation methods, rather than mapping an image or caption to a single point in the embedding space, represent elements of  $\mathcal{T}$ or $\mathcal{I}$ as random variables in $\widetilde{\mathcal{O}}$, thereby capturing the inherent one-to-many nature of the relationships.

However, the relationships among texts, images, and objects are inherently asymmetric, leading to distinct structures in text-to-image and image-to-text retrieval tasks. While both tasks are one-to-many, the asymmetry arises from different sources: abstraction and visual variability in text-to-image versus diverse textual descriptions in image-to-text. This structural difference motivates the use of asymmetric probabilistic structure for encoders within the representation space.

% \emph{From the uncertainty quantification (UQ) perspective}, aleatoric uncertainty arises from inherent randomness that cannot be reduced by additional data, while epistemic uncertainty stems from the model’s limited knowledge. Text carries high aleatoric uncertainty because a single label (e.g., "a dog") can refer to countless variations -- details like breed, size, or context being ambiguous. In contrast, images usually depict specific objects or scenes; a well-trained model can precisely identify them, given ample examples. However, if the training data lacks diversity, the model's epistemic uncertainty about an image will remain high, while aleatoric uncertainty will inherently be low.
\emph{From an uncertainty-quantification perspective}, we adopt the standard taxonomy of aleatoric vs. epistemic uncertainty \cite{hullermeier2021aleatoric}. Aleatoric uncertainty captures irreducible data ambiguity, e.g. the caption "a dog" denotes an entire class of breeds, poses and contexts, so no amount of additional training can pinpoint a single underlying object. Epistemic uncertainty captures model ignorance that could be reduced with more or better-distributed data, e.g., images, while depicting a unique scene with low aleatoric spread, may still suffer from coverage gaps if certain viewpoints or lighting conditions were under-represented during training. This asymmetry yields inherently broad aleatoric uncertainty in text versus more data‐dependent epistemic uncertainty in images. In practice, aleatoric uncertainty is modeled via parameterized distributions, whereas epistemic uncertainty is estimated by Monte Carlo methods (e.g., sampling from dropout layers or Bayesian neural networks). 
% Accordingly, in this work, focusing on aleatoric uncertainty, we represent text embeddings as directional distributions on the unit hypersphere and retain deterministic image vectors.

% good to make the text below softer
Assuming an underlying asymmetric uncertainty structure, a direction for improvement emerges. For text embeddings, it is essential to capture the wide variance inherent in language via distributions to reflect the multitude of corresponding objects. Conversely, image embeddings can be be modeled deterministically and the uncertainty is reduced through large coverage of visual data in the datasets.


==> asymvlm_latex/sec/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, our main claims made in the abstract and introduction are reflected by the paper's contributions through the experimental results in Section \ref{sec:results}.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The main limitations of the work, as well as future directions that may address some of these limitations, are discussed in Section \ref{sec:conclusion}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: Lemmas and theoretical results are well defined, and used to motivate and ground the proposed approach, with explicit assumptions and proofs as applicable.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The code for the paper is attached in the supplementary materials for the submission, and will be open-sourced through GitHub. The data for the paper is publicly available.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: All necessary details for experiments are provided in the Appendix.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All experiments were repeated five times with different random seeds, and we report the mean results in the main text, with full standard deviations provided in the Appendix.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All computing resources utilized for the experiments in the paper are listed in the Appendix.
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: This work does not entail any harmful consequences as laid out in the Code of Ethics.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Potential broader impacts of the paper are discussed in the main text. 
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: No such models or datasets are involved in the scope of this paper.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All code, data and models used in the paper are properly cited, and the license and terms of use are respected as specified.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The code for the paper is well documented with license, and terms of use being appended in the supplementary materials.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: No such models or datasets are involved in the scope of this paper.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: There are no human participants involved in the scope of this paper.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNo{}
    \item[] Justification: LLMs are not used for any important, original or non-standard component of the core methods.

\end{enumerate}


==> asymvlm_latex/sec/conclusion.tex <==
\section{Conclusion and limitation}\label{sec:conclusion}
% We have introduced AsymVLM, a novel post-hoc probabilistic adaptation framework for pretrained vision–language models that explicitly leverages the asymmetric uncertainty inherent in textual and visual embeddings. In AsymVLM, text embeddings are modelled as random variables parametrized by directional distributions on the unit hypersphere (e.g.\ von Mises–Fisher and power spherical), while image embeddings remain deterministic. By injecting these spherical likelihoods into an InfoNCE-style objective, AsymVLM jointly maximizes diagonal log-likelihoods and minimizes off-diagonals, effectively capturing wide‐variance aleatoric uncertainty in language.

% Extensive experiments on MS-COCO, Flickr-30k and Conceptual Caption (200k) show that AsymVLM variants consistently outperform both deterministic baselines and existing probabilistic methods in cross-modal retrieval (Recall@1) and produce more faithful uncertainty estimates. Ablation studies confirm the crucial roles of (i) the asymmetric adaptor architecture and (ii) spherical distribution modelling. Analysis on the HierarCap hierarchy further demonstrates that AsymVLM uncertainty aligns with linguistic abstraction, and applications in robust fine-tuning and “None-of-the-Above” zero-shot classification highlight its practical versatility.

We introduced AsymVLM, a post-hoc probabilistic adaptation framework for pretrained vision–language models that leverages asymmetric uncertainty in textual and visual embeddings. Text embeddings are modeled as random variables using directional distributions (e.g., von Mises–Fisher and power spherical) on the unit hypersphere, while image embeddings remain deterministic. Incorporating these spherical likelihoods into an InfoNCE-based objective enables effective modeling of wide-variance aleatoric uncertainty in language.

While AsymVLM delivers impressive performance in cross-modal retrieval with reliable uncertainty estimates, it only models text uncertainty. Future work could extend uncertainty modeling to image embeddings via data augmentation or similar methods. Also, although example applications of the uncertainty estimates are provided, further exploration into additional downstream tasks is warranted.

\section*{Broader impact}
Uncertainty estimates for text are vital in high-stakes applications involving VLMs, such as medical diagnostics where ambiguous language must be treated carefully. AsymVLM enhances trust in textual inputs, enabling safer and more robust applications of VLMs in uncertainty-sensitive domains.

\section*{Acknowledgement}
The computations/data handling were enabled by the Berzelius resource provided by the Knut and Alice Wallenberg Foundation at the National Supercomputer Centre, and by the Alvis resource provided by Chalmers e-Commons at Chalmers. LJ acknowledges funding from the Centre for Interdisciplinary Mathematics at Uppsala University and NAISS through Project 2024/22-1358. AH and PS acknowledge
support from the Swedish Research Council through grant agreement nos. 2023-05167 and 2023-05593 respectively. EV's research was partially supported by the
Kjell and Märta Beijer Foundation, and the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded by the Knut and Alice Wallenberg Foundation.
PS also acknowledges support from the the Knut and Alice Wallenberg foundation through the Program for Academic leaders in Life Science (PALS). 
The authors thank Aleksandr Karakulev, Csongor Horváth and Mayank Nautiyal for valuable discussions and feedback.


==> asymvlm_latex/sec/intro.tex <==

\section{Introduction}
\label{sec:intro}
Vision-language models (VLMs) have demonstrated impressive capabilities in understanding visual and linguistic information, by constructing a joint embedding space that aligns image and text embeddings \citep{vlm_intro, vlm_survey}. Models like CLIP \citep{clip} and BLIP \citep{blip}, enable a wide range of downstream applications, such as zero-shot classification \citep{clip_classification}, image-to-text retrieval \citep{cao2022image}, optical character recognition \citep{ocr}. However, due to the inherent ambiguity within text and image data, aligned point estimates for text and image embeddings produced by deterministic VLMs may not fully capture the complex relationships between the visual and linguistic embedding spaces. 

Alternatively, instead of learning deterministic point estimate embeddings, probabilistic embedding methods \citep{chun2021probabilistic} map text and language data onto probability distributions, more effectively capturing the ambiguity and uncertainty of the data. However, they entail training probabilistic VLMs from scratch on massive datasets -- an expensive process that forgoes the strengths of established deterministic VLMs. To explore post-hoc methods for constructing probabilistic embeddings from pretrained deterministic VLMs, recent frameworks such as ProbVLM \citep{probVLM_frozen_embeddings} and BayesVLM \citep{baumann2024post} have been proposed. However, the abmiguous nature of text-to-image retrieval is due to both textual abstraction and image variability, while image-to-text ambiguity arises from the multiplicity of textual descriptions. Existing methods overlook this asymmetric nature in texts and images, and the fact that the embeddings of most pre-trained VLMs reside on a unit hypersphere, instead of the Euclidean space. 

In this work, we propose a post-hoc method, Asymmetric Probabilistic Vision-Language Model (AsymVLM), to model the uncertainty of embeddings obtained from pretrained VLMs
\begin{itemize}[leftmargin=1.5em, itemsep=0.1em, topsep=0em]
    \item We formally address the asymmetric uncertainty structure inherent in vision–language data, high aleatoric uncertainty in text versus lower aleatoric uncertainty in images.
    \item We propose AsymVLM, an adapter that exploits the asymmetric uncertainty structure and performs post-hoc probabilistic adaptation on the unit hypersphere, rather than in Euclidean space. We also show that AsymVLM is a natural extension of CLIP’s cosine-similarity loss with the added ability to quantify uncertainty.
    \item Empirically, AsymVLM yields more accurate uncertainty estimates and higher cross-modal retrieval accuracy on multiple benchmarks. We further demonstrate its advantages in robust fine-tuning, zero-shot classification and "none-of-the-above" rejection. 
\end{itemize}
We formulate the problem, addressing the asymmetric structure of vision-language data in Section \ref{sec:asym}, and derive our method, AsymVLM, in Section \ref{sec:methods}. We then present empirical evaluations, including uncertainty quantification, ablation studies, and downstream applications in Section \ref{sec:results}. We conclude and discuss future work in Section \ref{sec:conclusion}.

\begin{figure}[t]
\vspace{1.1\shrinklength}
    \centering
    \includegraphics[width=\linewidth]{figures/comparison.pdf}
    \vspace{1.8\shrinklength}
    \caption{\textbf{Left}: Mapping relations between text, image, object, and representation spaces. \textbf{Right}: Comparison of methods -- CLIP uses deterministic one-to-one mappings; ProbVLM introduces one-to-many mappings via probabilistic embeddings; AsymVLM further captures asymmetry structure between texts, images and objects.}
    \label{fig:diagram}
    \vspace{\shrinklength}
\end{figure}

==> asymvlm_latex/sec/method.tex <==
\section{Method}\label{sec:methods}
With a pretrained VLM such as CLIP or SigLIP, we denote the text encoder as $f_T: \mathcal{T}\to\mathbb{S}^{d-1}$ and image encoder as $f_I: \mathcal{I}\to \mathbb{S}^{d-1}$, where $d$ is the dimension of the representation space. 

\subsection{Asymmetric probabilistic adaptation}
As discussed in Section \ref{sec:asym}, capturing the variance is crucial for text embeddings, while ensuring coverage in training data is key for image embeddings. To achieve this, we introduce a text adapter $g_T$ for the text encoder $f_T$, while retaining the deterministic embeddings from the image encoder $f_I$, as expanding image data coverage lies beyond the scope of this work.
Formally, the embedding of any text $t\in\mathcal{T}$ is modeled by a random variable $\bm{z}^T$,
\begin{align}
    \bm{z}^T \sim P(\theta(t)) \ \text{where}\ \theta(t) \coloneqq g_T \circ f_T(t)\label{eq:z_t},
\end{align}
where $P(\theta(t))$ denotes a distribution parametrized by $\theta(t)$ predicted by a neural network given corresponding text. The deterministic image embedding $z^I$ from the image encoder $f_I$ is retained.


\paragraph{Objective function} For any batch of data $\{(t_1, i_1), \dots, (t_B, i_B)\}$, we aim to maximize $\ln p_{\bm{z^T_n}}(z^I_n)$ for all $n\in[B]$ while minimizing $\ln p_{\bm{z}^T_m}(z^I_n)$ for all $n, m\in[B]$, $n\neq m$, where $p_{\bm{a}}(b)$ denotes the value of the PDF of random variable $\bm{a}$ at $b$. First we define the log likelihood matrix $L\in\mathbb{R}^{B\times B}$, where the $(m, n)$-th element is computed as $L(m, n) = \ln p_{\bm{z}^T_m}(z^I_n)$, for $n, m\in [B]$. 

To maximize the diagonal elements and minimize the off-diagonal elements of $L$, we apply the InfoNCE loss to $L$ and obtain the objective function to be minimized,
\begin{align}\label{eq:object}
    \underset{\theta\in\Theta}{\arg\min} -\frac{1}{2B} \sum_{n=1}^B
    \left [\ln \frac{ \exp{( \tau \cdot L(n, n))} }
    {\sum_{m=1}^B \exp{( \tau \cdot L(n, m))} }
    +
    \ln \frac{\exp{( \tau \cdot L(n, n))} }
    {\sum_{m=1}^B \exp{( \tau \cdot L(m, n))} }
    \right],
\end{align}
where $\tau$ is a temperature parameter and $\theta$ is the parameter set of distribution $P_{\bm{z}^T}(\theta(t))$.


\subsection{Modelling on the unit hypersphere}
The shared representation space built by most pre-trained VLMs is $\mathbb{S}^{d-1}$, the domain in which both $\bm{z}^T$ and $z^I$ reside. This observation necessitates the selection of a directional distribution for $P(\theta(t))$, defined on $\mathbb{S}^{d-1}$. To properly construct a probabilistic embedding on $\mathbb{S}^{d-1}$, directional distributions for the embeddings should be employed -- either projected distributions (e.g., the angular normal distribution) or native directional distributions (e.g., the vMF distribution). In this work, we use the vMF, and power spherical (PS) distributions to model the text embeddings distribution. The former is generally considered as the simplest directional distribution, while the latter is reported to be an alternative to the vMF distribution with a closed form normalization constant.

% However, both ProbVLM and BayesVLM overlook this aspect by selecting distributions on $\mathbb{R}^{d}$ to model the embeddings. Although the embeddings are first normalized and thereby projected onto the unit hypersphere, the likelihood calculations in their methods continue to employ distributions on $\mathbb{R}^d$. This approach neglects the probability mass of the dimension that is effectively collapsed by the projection. To properly construct a probabilistic embedding on $\mathbb{S}^{d-1}$, one should employ directional distributions for the projected embeddings, whether they are projected distributions (e.g., the angular normal distribution) or native directional distributions (e.g., the von Mises--Fisher distribution).

% In this work, we choose to use von Mises--Fisher (vMF) distribution and power spheric (PS) distribution to model the distribution of the text embeddings. The former one is generally considered as the simplest directional distribution in high dimensions, while the later is reported to be an alternative to vMF distribution with closed form normalization constant.

\paragraph{Derivation w.r.t. vMF distribution}
The vMF distribution $\operatorname{vMF}(\mu, \kappa)$ is a probability distribution on $\mathbb{S}^{d-1}$, parameterized by a mean direction $\mu\in\mathbb{R}^{d}$ and an isotropic concentration parameter $\kappa\in\mathbb{R}$, where $\lVert \mu\ \rVert_2 = 1$ and $\kappa \geq 0$. The PDF for random unit vector $x$ is given by,
\begin{align*}
    p(x; \mu, \kappa) = C_d(\kappa) \exp (\kappa \cdot \mu^\top x),
    \ \text{where} \ 
    C_d(\kappa) = \frac{\kappa^{d/2 - 1}}{(2\pi)^{d/2} I_{d/2 - 1}(\kappa)},
\end{align*}
and $I_p$ denotes the modified Bessel function of the first kind, at order $p$.

Following Equation \ref{eq:z_t}, assuming that $\bm{z}^T \sim \operatorname{vMF}(\mu(t), \kappa(t))$ for text $t\in\mathcal{T}$, for any image $i\in\mathcal{I}$, we have $\ln p_{\bm{z}^T}(z^I) = \kappa \cdot \mu(t)^\top z^I + \ln C_d(\kappa(t))$. However, computing $C_d(\kappa)$ is intractable in the high dimensional space, yet \cite{scott2021mises} have shown that $\ln C_d(\kappa)$ can be approximated by $F_d(\kappa) + \mathrm{const.}$,
where $F_d(\kappa)$ is given by,
{
\small
\begin{align*}
    F_d(\kappa) &=
    \frac{d-1}{4}\ln \left(\frac{d-1}{2} + \sqrt{\left( \frac{d-1}{2}\right)^2 + \kappa^2} \right) -\frac{1}{2}\sqrt{\left( \frac{d-1}{2}\right)^2 + \kappa^2}\\
    &+ \frac{d-1}{4}\ln \left(\frac{d-1}{2} + \sqrt{\left( \frac{d+1}{2}\right)^2 + \kappa^2}\right)
    - \frac{1}{2}\sqrt{\left( \frac{d+1}{2}\right)^2 + \kappa^2}.
\end{align*}
}
% By injecting the log likelihood of vMF into Equation \ref{eq:object}, we obtain the objective function to be minimized for vMF models as,
% \begin{align}
%     -\frac{1}{2B} \sum_{n=1}^B
%     \left [\ln \frac{ \exp{( \tau \cdot \mathrm{LL}_{\text{vMF}}(n, n) )} }
%     {\sum_{m=1}^B \exp{( \tau \cdot \mathrm{LL}_{\text{vMF}}(n, m) )} } 
%     +
%     \ln \frac{ \exp{( \tau \cdot \mathrm{LL}_{\text{vMF}}(n, n) )} }
%     {\sum_{m=1}^B \exp{( \tau \cdot \mathrm{LL}_{\text{vMF}}(m, n) )} }
%     \right],
% \end{align}
% where $\mathrm{LL}_{\text{vMF}}(r, s) = \kappa(t_r)\cdot \mu(t_r)^\top z^i_s + F_d(\kappa(t_r))$.

Injecting the log likelihood of vMF into Equation \ref{eq:object} results in the vMF kernel for the objective function $L_{\text{vMF}}$ as follows,
\begin{align*}
    L_{\text{vMF}}(r, s) = \kappa(t_r)\cdot \mu(t_r)^\top z^I_s + F_d(\kappa(t_r)), \ \forall r, s\in[B].
\end{align*}

The detailed derivation for the approximation is deferred to Appendix \ref{app:approx}.


\paragraph{Derivation w.r.t. PS distribution}
The power spheric distribution $\operatorname{PS}(\mu, \kappa)$ is an alternative to vMF, also parametrized by a mean direction $\mu\in\mathbb{R}^{d}$ and a concentration parameter $\kappa \in \mathbb{R}$ with $\lVert \mu\rVert_2=1$ and $\kappa \geq 0$. The PDF of a PS distribution is given by,
\begin{align*}
    p(x; \mu, \kappa) = (1+\mu^\top x)^\kappa \cdot C_d(\kappa),
    \  \text{where} \ 
    C_d(\kappa) = \left\{2^{\alpha + \beta} \pi^\beta \frac{\Gamma(\alpha)}{\Gamma(\alpha + \beta)} \right\}^{-1},
\end{align*}
and $\alpha = (d-1)/2+\kappa, \beta = (d-1)/2$.

%where $\alpha = \frac{d-1}{2}+\kappa$ and $\beta = \frac{d-1}{2}$.

Similarly, following Equation \ref{eq:z_t}, assuming that $\bm{z}^t \sim \operatorname{PS}(\mu(t), \kappa(t))$ for text $t\in\mathcal{T}$, for any image $i\in\mathcal{I}$, injecting the log likelihood of PS distribution in Equation \ref{eq:object} results in the PS kernel $L_{\text{PS}}$,
{
\small
\begin{align*}
L_{\text{PS}}(r, s) =& \kappa(t_r)\ln(1+\mu(t_r)^\top z^I_s) - (d-1+\kappa(t_r))\ln 2 \\
-& \ln \Gamma\left(\frac{d-1}{2}+\kappa(t_r)\right) + \ln \Gamma(d-1+\kappa(t_r)), \ \forall r, s\in [B].
\end{align*}
}
% \begin{align}
%     -\frac{1}{2B} \sum_{n=1}^B
%     \left [\ln \frac{ \exp{( \tau \cdot \mathrm{LL}_{\text{PS}}(n, n) )} }
%     {\sum_{m=1}^B \exp{( \tau \cdot \mathrm{LL}_{\text{PS}}(n, m) )} }
%     +
%     \ln \frac{ \exp{( \tau \cdot \mathrm{LL}_{\text{PS}}(n, n) )} }
%     {\sum_{m=1}^B \exp{( \tau \cdot \mathrm{LL}_{\text{PS}}(m, n) )} }
%     \right],
% \end{align}
% where the closed form of the log likelihood is given by,
% \begin{align*}
% \mathrm{LL}_{\text{PS}}(r, s) = \kappa(t_r)\ln(1+\mu^\top z^i_s) - (d-1+\kappa(t_r))\ln 2 
% - \ln \Gamma\left(\frac{d-1}{2}+\kappa(t_r)\right) + \ln \Gamma(d-1+\kappa(t_r)).
% \end{align*}

\subsection{Uncertainty quantification}
% how aleatoric uncertainty is quantified: show the concentration parameter is a good measure of aleatoric uncertainty
We quantify text‐embedding uncertainty as $u(t)=1/\kappa(t)$, due to the fact that for both the vMF and PS distributions on $\mathbb{S}^{d-1}$, the (angular) variance $\sigma^2$ is a strictly decreasing function of $\kappa$. Equivalently, larger $\kappa$ concentrates mass more tightly around the mean direction (lower $\sigma^2$), so $1/\kappa$ grows monotonically with the distribution’s variance, providing a natural scalar value for uncertainty estimate for probabilistic embeddings.

\subsection{Connections to CLIP}
Equation \ref{eq:object} can be rewritten in the following form,
\begin{align*}
    \theta = \underset{\theta\in\Theta}{\arg\min} -\frac{1}{2B} \sum_{n=1}^B
    \left[\ln \frac{ \exp{( \tau \delta(n, n) )} }
    {\sum_{m=1}^B \exp{( \tau \delta(n, m) )} } 
    +
    \ln \frac{\exp{( \tau \delta(n, n) )} }
    {\sum_{m=1}^B \exp{( \tau \delta(m, n) )} }
    \right].
\end{align*}
Denoting $\operatorname{CosSim}(r,s) = \mu(t_r)^\top z_s^I$, for any $r, s\in[B]$ we have,
\begin{equation}\label{eq:unified_form}
\begin{aligned}
&\text{for CLIP: } \delta_{\text{CLIP}}(r, s) = \operatorname{CosSim}(r,s),\\
&\text{for AsymVLM$_{\operatorname{vMF}}$: } \delta_{\text{vMF}}(r, s) = \kappa(t_r)\cdot \operatorname{CosSim}(r,s) + F_d(\kappa(t_r)),\\
&\text{for AsymVLM$_{\operatorname{PS}}$: } \delta_{\text{PS}}(r, s) = \kappa(t_r)\ln(1+\operatorname{CosSim}(r,s) + \ln C_d(\kappa(t_r)).
\end{aligned}
\end{equation}

Given that $\kappa(t_r)\geq 0$, it is clear that the latter two objectives are monotonically increasing w.r.t. $\delta_{\text{CLIP}}$ with an additional parameter $\kappa$. These can be interpreted as \emph{extensions of the CLIP loss by introducing $\kappa$, the concentration parameter, to model the variance of the text embedding without drifting from the pre-trained models using cosine similarities}.


\begin{mdframed}
Equation \ref{eq:unified_form} demonstrates AsymVLM's consistency with the underlying ideas of CLIP, while incorporating mechanisms to account for embedding variance. AsymVLM ultimately offers a more refined and probabilistically grounded approach to modeling semantic relationships between text and images. Furthermore, AsymVLM can be extended to a SigLIP variant. Inference using AsymVLM also extends beyond simply computing the cosine similarity, to utilizing the maximum likelihood principle, with a clearer statistical explanation. Details about the inference process and its SigLIP-variant are provided in Appendix \ref{appen:inference} and \ref{appen:siglip}.    
\end{mdframed}


% \subsection{Inference with maximum log likelihood}
% The inference of deterministic pre-trained VLMs (i.e. cross-modal retrieval) replies on computing the cosine similarities of each possible pairs of given texts and images, while the inference for AsymVLM has a clear statistical interpretation as maximizing log likelihood w.r.t. different image-text pairs. For Image-to-Text retrieval, given a set of text embeddings $\{\bm{z}^t_r \vert r\in[R]\}$, where $\bm{z}^t_r \sim \operatorname{vMF}(\mu_r^t, \kappa_r^t)$ or $\bm{z}^t_r \sim \operatorname{PS}(\mu_r^t, \kappa_r^t)$, and an image embeddings $z^i$, the predictor is given by,
% \begin{align*}
%     \hat{r} = \underset{r\in[R]}{\arg}\max \ln p_{\bm{z}^t_r}(z^i)=
%     \begin{cases}
%     \kappa^t_r \cdot (\mu^t_r)^\top z^i  + F_d(\kappa^t_r) & \text{for vMF},\\
%     \kappa^t_r\ln(1+ (\mu^t_r))^\top z^i + \ln C_d(\kappa^t_r) & \text{for PS}.
%     \end{cases}
% \end{align*}
% Similarly, for Text-to-Image retrieval, given a set of image embeddings $\{z^i_s \vert s\in[S]\}$ and a text embedding $\bm{z^t}\sim \operatorname{vMF}(\mu^t, \kappa^t)$ or $\bm{z^t}\sim \operatorname{PS}(\mu^t, \kappa^t)$, the predictor is given by,
% \begin{align*}
%     \hat{s} = \underset{s\in[S]}{\arg}\max \ln p_{\bm{z}^t}(z^i_s)=
%     \begin{cases}
%     \kappa^t \cdot (\mu^t)^\top z^i_s  + F_d(\kappa^t) & \text{for vMF},\\
%     \kappa^t \ln(1+ (\mu^t)^\top z^i_s + \ln C_d(\kappa^t) & \text{for PS}.
%     \end{cases}
% \end{align*}


==> asymvlm_latex/sec/related.tex <==
\section{Related work}\label{sec:related}
\paragraph{Vision-language models}
%Recent advances in vision-language modeling enable multimodal models to learn a shared embedding space for images and text, often by optimizing directional similarity metrics (e.g., cosine similarity). 
Recent advancements in vision-language modeling have facilitated the development of multimodal models capable of learning a shared embedding space for images and text. These models typically achieve this by optimizing directional similarity metrics, such as cosine similarity. Notable works including CLIP \cite{clip}, BLIP \cite{blip}, SigLIP \cite{zhai2023sigmoid}, typically align paired image-text representations by maximizing the cosine similarity between corresponding embeddings. This strategy has proven to be effective for large-scale training, enabling these models to capture semantic relationships, and generalize well across diverse downstream tasks. However, these pretrained VLMs offer deterministic mappings that fail to capture the inherent ambiguity in the inputs.

\paragraph{Probabilistic VLMs}
Methods have been proposed to improve deterministic VLM embeddings by learning a unified probabilistic embedding space for both visual and textual data. Methods such as PCME \cite{chun2021probabilistic}, and PFE \cite{shi2019probabilistic} learn to map texts and images to aligned probability distributions, by maximizing the cross-modal likelihood between corresponding text and image data. However, these approaches require training from scratch, which is computationally expensive as existing high-quality deterministic VLMs are not fully leveraged. A more resource-efficient alternative is the probabilistic adaptation of pretrained VLMs. ProbVLM \cite{probVLM_frozen_embeddings} trains an adapter to construct probability distributions from deterministic embeddings, while BayesVLM \cite{baumann2024post} estimates the uncertainty of cosine similarity through post-hoc Bayesian posterior approximation. As mentioned in Section \ref{sec:intro} (and detailed in the following Section), although having demonstrated their efficacy for uncertainty quantification, existing post-hoc approaches do not consider the asymmetry in uncertainty structures between textual and visual data, and the constraint that meaningful embeddings of most pretrained VLMs reside on the unit sphere, resulting in sub-optimal performance.

\paragraph{Embeddings on the unit hypersphere}
Cosine similarity is widely utilized in contemporary VLMs and foundation models pre-trained with contrastive loss \cite{chen2020simple, clip, chen2021exploring}. This approach inherently constrains the learned embeddings to reside on the unit hypersphere. These embeddings have been shown to have advantages such as improved uniformity and alignment compared to their Euclidean counterparts \cite{pmlr-v119-wang20k}. Beyond cosine similarity, embeddings on the unit hypersphere can also be explicitly modeled by assuming directional distributions, such as the von Mises-Fisher (vMF) distribution \cite{dhillon2003modeling}. \citet{scott2021mises} introduced a contrastive loss based on the vMF distribution as a pretraining method, while \cite{sandhuclip} proposes a method to distill pretrained VLMs, adapting student models with vMF assumptions for zero-shot classification. However, while these approaches focus on improving empirical performance in downstream tasks, none explicitly model the uncertainty of embeddings from pretrained VLMs.



==> asymvlm_latex/sec/result.tex <==
\section{Empirical results}\label{sec:results}
We compare AsymVLM to the baselines on benchmark datasets, and subsequently present an ablation study. Further, extended analyses and demonstration on two downstream applications are presented.

\paragraph{Datasets, baselines and metrics} The MS-COCO \cite{coco_dataset} and Flickr-30k \cite{flickr_dataset} datasets are used to train the adapters. Additionally, a subset of the Conceptual Caption dataset \cite{sharma2018conceptual} of 200k samples (CC-200k) is also used. To understand the nature of learned uncertainty, the HierarCap dataset \cite{alper2024emergent} is used, containing four captions of different abstraction levels for each image. The baselines include BayesVLM, ProbVLM, ProLIP, PFE and PCME++ adapted from pretraining methods (denoted by $\text{PFE}^\star$ and $\text{PCME++}^\star$, respectively). The pre-trained VLM used in the experiments in the main text is CLIP (ViT-B/32 backbone). We assess the uncertainty quality in text embeddings by evaluating recall@1 performance in cross-modal retrieval tasks. A strong positive correlation between uncertainty and errors indicates that higher uncertainty leads to poorer embeddings and lower recall. For each task, we group results by uncertainty levels and compute Spearman's rank correlation ($S$) between uncertainty and recall \cite{sedgwick2014spearman}. We then fit a regressor ($R^2$) to determine if the performance drop is linear, and compare average Recall@1 across uncertainty levels for different methods. All experiments were repeated \emph{five times with different random seeds}, and we report the mean results with full standard deviations provided in the Appendix. The code for this paper is available at \url{https://github.com/li-ju666/asymvlm}.

\subsection{Evaluation of UQ and cross-modal retrieval}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.325\linewidth]{figures/results/uncertainty/coco.pdf}
    \includegraphics[width=0.325\linewidth]{figures/results/uncertainty/flickr.pdf}
    \includegraphics[width=0.325\linewidth]{figures/results/uncertainty/cc.pdf}
    % \vspace{0.5\shrinklength}
    \caption{Recall@1 versus uncertainty levels for cross-modal retrieval tasks for various datasets. Each subplot shows the performance degradation as uncertainty increases for $\text{PFE}^\star$, $\text{PCME++}^\star$, ProbVLM, $\text{AsymVLM}_\text{vMF}$, and $\text{AsymVLM}_\text{PS}$. Ideally Recall@1 should decrease monotonically.}
    \label{fig:unc_ret}
    \vspace{\shrinklength}
\end{figure}

\vspace{-\shrinklength}
\begin{table}[ht]
\scriptsize
\centering
\caption{Evaluation of model performance and uncertainty on benchmarks (MS-COCO, Flickr-30k, CC-200k) for Image-to-Text (i2t) and Text-to-Image (t2i) retrieval. We report Recall@1 $\uparrow$, regression fit $R^2 \uparrow$ between uncertainty and retrieval error, and Spearman’s rank $S\downarrow$ correlation between uncertainty and retrieval error. \textbf{Bold} font denotes the best results and \underline{underline} denotes the second best results. Each value is the mean of 5 runs with standard deviation in the Appendix, Table \ref{app_tab:unc_ret_clip}.}
\label{tab:unc_ret}
\vspace{0.5em}
\begin{tabular}{ll ccc ccc}
\toprule
& & \multicolumn{3}{c}{\textbf{\textsc{t2i}}} & \multicolumn{3}{c}{\textbf{\textsc{i2t}}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
\textbf{\textsc{Dataset}} & \textbf{\textsc{Method}} & Recall@1 $\uparrow$ & $R^2\uparrow$  & $S\downarrow$ & Recall@1 $\uparrow$ & $R^2\uparrow$  & $S\downarrow$ \\
\midrule

& $\text{PFE}^\star$ &0.500 &0.558 &-0.722 &0.304 &0.946 &-0.988 \\
& $\text{PCME++}^\star$ &0.500 &0.931 &\textbf{-0.996} &0.304 &0.948 &-0.990 \\
& $\text{BayesVLM}$ &0.506 &0.884 &-0.976 &0.323 &0.932 &-0.985 \\
\textbf{\textsc{MS-COCO}}
& $\text{ProbVLM}$  &0.480 &\textbf{0.951} &-0.981 &0.293 &0.979 &\textbf{-1.000} \\
& $\text{ProLip}$  &0.500 &0.808 &-0.908 &0.304 &0.876 &-0.985 \\
& $\text{AsymVLM}_{\text{vMF}}$ &\textbf{0.561} &\underline{0.948} &\underline{-0.988} &\textbf{0.392} &\underline{0.984} &\textbf{-1.000} \\

& $\text{AsymVLM}_{\text{PS}}$ &\underline{0.558} &0.937 &-0.984 &\underline{0.390} &\textbf{0.989} &\textbf{-1.000} \\
\midrule

& $\text{PFE}^\star$ &0.680 &0.675 &-0.832 &0.451 &0.955 &\textbf{-0.998} \\
& $\text{PCME++}^\star$ &0.679 &0.455 &-0.178 &0.451 &0.900 &-0.918\\
& $\text{BayesVLM}$ &0.637 &\textbf{0.916} &\textbf{-0.976} &0.425 &0.934 &-0.973\\
\textbf{\textsc{Flickr-30k}}
& $\text{ProbVLM}$  &0.646 &0.826 &-0.914 &0.422 &\textbf{0.964} &-0.985 \\
& $\text{ProLip}$  &0.678 &0.829 &-0.954 &0.450 &0.928 &-0.978 \\
& $\text{AsymVLM}_{\text{vMF}}$ &\textbf{0.688} &\underline{0.860} &\textbf{-0.976} &\textbf{0.504} &\underline{0.960} &\underline{-0.995} \\

& $\text{AsymVLM}_{\text{PS}}$ &\textbf{0.688} &0.854 &-0.947 &\underline{0.498} &0.946 &-0.993 \\
\midrule

& $\text{PFE}^\star$ &0.352 &0.857 &-0.521 &0.336 &0.988 &-0.595 \\
& $\text{PCME++}^\star$ &0.352 &0.198 &-0.148 &0.336 &0.779 &-0.887 \\
& $\text{BayesVLM}$ &0.347 &0.905 &-0.968 &0.304 &0.874 &-0.937\\
\textbf{\textsc{CC-200k}}
& $\text{ProbVLM}$   &0.316 &0.772 &-0.837 &0.302 &0.775 &-0.965 \\
& $\text{ProLip}$  &0.351 &0.968 &-0.990 &0.335 &\underline{0.992} &\textbf{-1.000} \\
& $\text{AsymVLM}_{\text{vMF}}$  &\textbf{0.395} &\underline{0.990} &\textbf{-1.000} &\textbf{0.383} & 0.991 & -0.998 \\
& $\text{AsymVLM}_{\text{PS}}$ &\underline{0.393} &\textbf{0.992} &\textbf{-1.000} &\underline{0.380} &\textbf{0.993} &\textbf{-1.000} \\
\bottomrule
\vspace{\shrinklength}
\end{tabular}
\end{table}

Figure~\ref{fig:unc_ret} and Table~\ref{tab:unc_ret} summarize the main results comparing the proposed AsymVLM with baseline methods. For uncertainty quantification, results indicate that while all methods capture text uncertainty to some degree, AsymVLM consistently outperforms its counterparts. As the uncertainty level increases, AsymVLM is the only method for which Recall@1 decreases strictly monotonically. Moreover, AsymVLM also meets or exceeds competing approaches on both \(R^2\) and \(S\) scores.

In cross-modal retrieval, $\text{AsymVLM}_{\text{vMF}}$ and $\text{AsymVLM}_{\text{PS}}$ achieve the highest and second-highest Recall@1 scores across all datasets. Note that the retrieval performances of $\text{PFE}^\star$ and $\text{PCME++}^\star$ are identical, as they only model the variance of embeddings while while keeping embedding directions constant, resulting in performance identical to the pre-trained models. In contrast, both AsymVLM and ProbVLM adapt the directions and learn the uncertainty of the embeddings during post-hoc training. Although ProbVLM achieves reasonable uncertainty estimates overall, it consistently under-performs pre-trained models in recall, whereas AsymVLM delivers richer uncertainty estimates and improves cross-modal retrieval performance.

Furthermore, the similar performance of $\text{AsymVLM}_{\text{vMF}}$ and $\text{AsymVLM}_{\text{PS}}$ in both cross-modal retrieval and uncertainty quantification shows the robustness of AsymVLM w.r.t. the choice of the spherical distribution, suggesting possibilities of exploring other spherical or directional distributions.

\subsection{Ablation study}
We conduct an ablation study on the two important components of AsymVLM: the asymmetric architecture of the adapter, and the use of a spherical distribution for modeling. To assess the impact of two components, we designed following adapters with experimental results presented in Figure \ref{fig:ablation}:
\begin{itemize}[leftmargin=1.5em, itemsep=0.1em, topsep=0em]
    \item \textbf{AsymVLM(image):} This variant modifies AsymVLM by only mapping deterministic image embeddings to spherical distributions, leaving text embeddings deterministic.
    \item \textbf{SymVLM:} This variant map both deterministic image and text embeddings to spherical distributions, with InfoNCE applied to symmetrized log likelihood kernel.
    \item \textbf{AsymVLM($\mathcal{G}$):} This variant has identical architecture with AsymVLM but maps deterministic text embedding on Gaussian distribution, followed by normalization. The kernel of the loss function is replaced by Gaussian log likelihood.
\end{itemize}

\paragraph{Asymmetric architecture}
Both AsymVLM(image) and SymVLM perform worse than the original AsymVLM with respect to uncertainty quantification. Specifically, AsymVLM(image) struggles to model image uncertainty, showing no decrease in Recall@1 as uncertainty increases. Although SymVLM exhibits a slight decrease in Recall@1 with rising uncertainty, uncertainty estimates remain sub-optimal to AsymVLM. AsymVLM(image) achieves average Recall@1 comparable to AsymVLM while SymVLM performs much worse than either AsymVLM or AsymVLM(image). The results underscore the importance of an asymmetric architecture for uncertainty quantification and cross-modal retrieval performance.

\paragraph{Choice of spherical distributions}
For both Image-to-Text and Text-to-Image retrieval tasks, $\text{AsymVLM}(\mathcal{G})$ yields reasonable uncertainty estimates. As uncertainty levels increase, the Recall@1 of $\text{AsymVLM}(\mathcal{G})$ declines almost linearly, exhibiting behaviour similar to AsymVLM. However, the overall Recall@1 is inferior compared to AsymVLM. This emphasizes not only the effectiveness of the asymmetric architecture for uncertainty quantification, but also the necessity of spherical distributions for the post-hoc adaptation of pre-trained VLMs.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/results/ablation.pdf}
    % \vspace{1.2\shrinklength}
    \caption{Ablation study results for AsymVLM: The left and middle panel shows Recall@1 performance for cross-modal retrieval across various uncertainty levels. The right panel summarizes average Recall@1 for both retrieval tasks.}
    \label{fig:ablation}
    \vspace{\shrinklength}
\end{figure}

\subsection{Understanding the uncertainty estimates}
To better understand the uncertainty estimates produced by AsymVLM, we analyze caption estimates on the HierarCap dataset. In this dataset, each image is paired with hierarchical captions spanning four levels -- from general descriptions (Level 0) to detailed image descriptions (Level 3). Figure \ref{fig:unc_study} illustrates the following observations.

\begin{itemize}[leftmargin=1.5em, itemsep=0.1em]
    \item \textbf{AsymVLM captures hierarchical caption structure} Level 0 captions with general descriptions exhibit higher uncertainty estimates, indicating greater ambiguity, while Level 3 captions with the most detail generally show lower uncertainty. This pattern aligns with the inherent ambiguity of language and the corresponding uncertainty estimates provided by AsymVLM.
    
    \item \textbf{Detailed captions enhance image retrieval likelihood} The likelihood of the image embedding increases as more detailed descriptions are provided, as shown by the shift towards higher log likelihood values from Level 0 to 3. This suggests that detailed captions better capture the nuances of the image, facilitating more accurate image retrieval.

    \item \textbf{Longer captions exhibit reduced ambiguity} The results indicate that a higher token count is associated with lower uncertainty in the text, as depicted by the downward trend in uncertainty values. This is aligned with the expectation, as shorter texts generally tend to be more ambiguous, while longer captions provide more context, reducing ambiguity.
\end{itemize}
% \paragraph{AsymVLM captures hierarchical caption structure} Captions with general descriptions (Level 0) exhibit higher uncertainty estimates, indicating greater ambiguity, while captions at Level 4, which contain the most detail, generally show lower uncertainty. This pattern aligns with the inherent ambiguity of language and the corresponding uncertainty estimates provided by AsymVLM.

% \paragraph{Detailed captions enhance image retrieval likelihood} Despite each image having four associated captions, the likelihood of the image embedding increases as more detailed descriptions are provided, as shown by the shift towards higher log likelihood values from Level 0 to Level 3. This suggests that detailed captions better capture the nuances of the image, facilitating more accurate image retrieval.

% \paragraph{Longer captions exhibit reduced ambiguity} The results indicate that a higher token count is associated with lower uncertainty in the text, as depicted by the downward trend in uncertainty values. This is aligned with the expectation, as shorter texts generally tend to be more ambiguous, while longer captions provide more context, reducing ambiguity.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/results/unc_study.pdf}
    \vspace{1.2\shrinklength}
    \caption{Uncertainty and likelihood analysis with the HierarCap dataset. The left panel shows the distribution of uncertainty estimates across hierarchical caption levels, showing decreasing uncertainty from Level 0 to 3. The middle panel illustrates the log likelihood distribution of image embeddings, with increased likelihood as caption detail increases. The right panel shows the relationship between the number of tokens and uncertainty, indicating reduced uncertainty with longer captions.}
    \label{fig:unc_study}
    \vspace{\shrinklength}
\end{figure}

\subsection{Applications}\label{sec:res_app}
Below, we present two example applications of the uncertainty estimates obtained from AsymVLM, demonstrating their potential use cases.

\paragraph{Handling none-of-the-above}
\begin{wraptable}{r}{0.52\textwidth}
\vspace{\shrinklength}
\scriptsize
  \centering
  \caption{None-of-the-above-aware zero-shot classification using dummy prompts. The table reports the accuracy on positive samples and negative samples.}
  \begin{tabular}{llcc}
    \toprule
    \textbf{\textsc{Dummy Class}} & \textbf{\textsc{Method}} & \textbf{\textsc{Pos. Acc.}} & \textbf{\textsc{Neg. Acc.}} \\
    \midrule
    \multirow{3}{*}{\texttt{"a photo"}} 
      & CLIP & \textbf{0.888} & 0.009 \\
      & Determ. FT & 0.769 & 0.115\\
      & $\text{AsymVLM}_{\text{PS}}$ 
      & 0.845 & \underline{0.547}\\
      & $\text{AsymVLM}_{\text{vMF}}$
      & \underline{0.857} & \textbf{0.587}\\

    \midrule
    \multirow{4}{*}{\shortstack{\texttt{"a photo of} \\ \texttt{an object"}}} 
      & CLIP & \textbf{0.888} & 0.009 \\
      & Determ. FT & 0.778 & 0.037\\
      & $\text{AsymVLM}_{\text{PS}}$ 
      & 0.849 & \textbf{0.609}\\
      & $\text{AsymVLM}_{\text{vMF}}$
      & \underline{0.858} & \underline{0.557}\\

    \midrule
    \multirow{4}{*}{\shortstack{\texttt{"a photo of} \\ \texttt{something"}}} 
      & CLIP & \textbf{0.888} & 0.009 \\
      & Determ. FT & 0.769 & 0.125\\
      & $\text{AsymVLM}_{\text{PS}}$ 
      & 0.843 & \textbf{0.595}\\
      & $\text{AsymVLM}_{\text{vMF}}$
      & \underline{0.857} & \underline{0.585}\\
    \midrule
    \multirow{2}{*}{\textbf{\textsc{None}}} 
      & Margin-Based & 0.584 & 0.579 \\
      & Threshold-Based & 0.646 & 0.560 \\
    \bottomrule

  \vspace{1.5\shrinklength}
  \end{tabular}
  \label{tab:robust_zs}
\end{wraptable}

For zero-shot classification, strategies to enable a model to say \texttt{"none-of-the-above"} rather than assigning an incorrect label include threshold-based rejection, margin-based rejection and other techniques. AsymVLM provides an alternative approach, by introducing a dummy prompt such as \texttt{"a photo"} to signal \texttt{"none-of-the-above"}. We evaluate these methods on a combined test set consisting of CIFAR-10 and CIFAR-100 samples, performing zero-shot classification over CIFAR-10 classes. Ideally, CIFAR-10 samples (positive samples) should be correctly classified into their respective categories, while CIFAR-100 samples (negative samples) should be rejected as \texttt{"none-of-the-above"}. AsymVLM consistently outperforms other methods (Table~\ref{tab:robust_zs}), achieving higher accuracy on both positive and negative samples.

\paragraph{Robust fine-tuning}
% \begin{wraptable}{r}{0.59\textwidth}
% \vspace{\shrinklength}
\begin{table}[ht]
\scriptsize
  \centering
  \caption{Zero‐shot classification accuracy. "None" denotes the baseline without fine‐tuning.}

  \begin{tabular}{llcccc}
    \toprule
    & & \multicolumn{4}{c}{\textbf{\textsc{Validated on}}} \\
    \cmidrule(lr){3-6}

    \textbf{\textsc{Fine-Tuned}} & \textbf{\textsc{Method}} & \textbf{\textsc{CIFAR-10}} & \textbf{\textsc{CIFAR-100}} & \textbf{\textsc{STL-10}} & \textbf{\textsc{ImageNet-1k}}\\
    \midrule
    \multirow{3}{*}{\textbf{\textsc{MS-COCO}}} 
      & Determ. FT
      &0.684 &0.300 &0.829 & 0.395\\
      & $\text{AsymVLM}_{\text{PS}}$
      &\textbf{0.847}  &\underline{0.470}  &\textbf{0.952} & \underline{0.502} \\
      & $\text{AsymVLM}_{\text{vMF}}$
      &\underline{0.837} &\textbf{0.477} &\underline{0.940} & \textbf{0.507} \\

    \midrule
    \multirow{3}{*}{\textbf{\textsc{Flickr-30k}}} 
      & Determ. FT
      &0.688 &0.342 &0.874 & 0.369\\
      & $\text{AsymVLM}_{\text{PS}}$
      &\underline{0.791} &\underline{0.413} &\textbf{0.920} & \underline{0.451}\\
      & $\text{AsymVLM}_{\text{vMF}}$
      &\textbf{0.792} &\textbf{0.422} &\underline{0.918} & \textbf{0.464}\\

    \midrule
    \multirow{3}{*}{\textbf{\textsc{CC-200k}}} 
      & Determ. FT
      &0.779  &0.411  &0.922 & 0.450\\
      & $\text{AsymVLM}_{\text{PS}}$
      &\underline{0.861} &\textbf{0.542}  &\textbf{0.968}  & \underline{0.520}\\
      & $\text{AsymVLM}_{\text{vMF}}$
      &\textbf{0.866} &\textbf{0.542}  &\underline{0.967} & \textbf{0.527} \\
      \midrule
      \multirow{1}{*}{\textbf{\textsc{None}}} 
      & CLIP & 0.888 & 0.642 & 0.974 & 0.632\\
    \bottomrule
  % \vspace{1.5\shrinklength}
  \end{tabular}
  \label{tab:zero_shot}
% \end{wraptable}
\end{table}
Pre-trained VLMs are renowned for their zero-shot classification performance. However, fine-tuning these models on smaller datasets typically impairs this capability on other datasets. Table~\ref{tab:zero_shot} compares AsymVLM with its deterministic counterpart, denoted by Determ.FT, and the foundation model without fine-tuning. Models fine-tuned with AsymVLM consistently outperform those fine-tuned deterministically across all settings. This suggests that AsymVLM preserves the zero-shot classification proficiency acquired during pre-training to a greater extent, whereas the deterministic approach is more prone to catastrophic forgetting. Therefore, AsymVLM offers a more robust fine-tuning strategy for VLMs.


% Although margin- and threshold-based methods can reach comparable rejection performance with careful hyperparameter tuning, their accuracy on positive samples drops. This demonstrates that AsymVLM provides a robust and effective solution for zero-shot classification with reliable "None of the Above" handling.
